Influence Patterns for Explaining Information Flow in BERT

While attention is all you need may be proving true, we do not know why: attention-based transformer models such as BERT are superior but how information flows from input tokens to output predictions are unclear. We introduce influence patterns, abstractions of sets of paths through a transformer model. Patterns quantify and localize the flow of information to paths passing through a sequence of model nodes. Experimentally, we find that significant portion of information flow in BERT goes through skip connections instead of attention heads. We further show that consistency of patterns across instances is an indicator of BERT's performance. Finally, We demonstrate that patterns account for far more model performance than previous attention-based and layer-based methods.

==> Makefile <==
OS   := $(shell uname)
ifeq ($(OS), Linux)
  OPEN := evince
else
ifneq ("$(wildcard /Applications/Skim.app)","")
  OPEN := open -a /Applications/Skim.app
else
  OPEN := open -a /Applications/Preview.app
endif
endif
DOC  := doc-inflgraph
MAIN := main
PDFLATEX := pdflatex

DEP_FIGS := $(shell find ./figures \
	-name '*.tex' \
	)
DEP := *.tex *.bib $(DEP_FIGS)
DEP := $(foreach i,$(DEP),$(shell ls $(i) 2> /dev/null))

start:
	make draft

start-%:
	make open-$*
	make watch-$*

draft:
	make start-draft

final:
	make start-final

$(DOC).final.main.pdf: $(DOC).final.pdf
	pdftk $(DOC).final.pdf cat 1-9 output $@

$(DOC).final.supplemental.pdf: $(DOC).final.pdf
	pdftk $(DOC).final.pdf cat 10-12 output $@

parts: $(DOC).final.main.pdf $(DOC).final.supplemental.pdf

startt:
	$(PDFLATEX) $(QUIET) preamble; $(BIBTEX) $(QUIET) $(MAIN); $(PDFLATEX) $(QUIET) preamble; $(PDFLATEX) $(QUIET) preamble;
	make clean; $(OPEN) preamble.pdf

open-%: $(DOC).%.pdf
ifneq ("$(OPEN)","")
	$(OPEN) $(DOC).$*.pdf ; sleep 1
else
	@echo "Could not find a PDF reader. If you'd like this \
	makefile to open the generated pdfs, add your PDF reader to \
	the opening section of the Makefile."
	@exit 1
endif

$(DOC).pdf: $(DEP)
	perl watch.pl render_latex $(MAIN) "\input{$(MAIN).tex}" $(DOC)
#	@cp $(MAIN).pdf $(DOC).pdf
#	@cp $(MAIN).synctex.gz $(DOC).synctex.gz


$(DOC).%.pdf: $(DEP)
	perl watch.pl render_latex $(MAIN) "\def\$*{}\input{$(MAIN).tex}" $(DOC).$*
#	@cp $(MAIN).pdf $(DOC).$*.pdf
#	@cp $(MAIN).synctex.gz $(DOC).$*.synctex.gz

watch-%:
	perl watch.pl watch $(DOC).$*.pdf $(DEP)
	perl watch.pl watch $(DOC).pdf $(DEP)

# DEBUGGING UTILS
# https://www.cmcrossroads.com/article/printing-value-makefile-variable
print-%  : ; @echo $* = $($*)

debug: $(DEP)
	$(PDFLATEX) -interaction nonstopmode "\input{$(MAIN).tex}"
	$(OPEN) $(DOC).pdf

# To debug unicode issues:
# useful emacs command: find-file-literally
show_unicode: $(DEP)
	pcregrep --color='auto' -n "[\x80-\xFF]" *.tex *.bib

# List all references to the thing after find_ in the tex sources.
find_%: *.tex
	grep -I -C 1 -n --color=auto '$*' *.tex; true

# CLEANING
clean:
	rm -Rf *.aux *.lof *.log *.lot *.bbl *.blg *.toc *.out *.bcf *.run.xml; true
	rm -Rf *~; true
	rm -Rf $(DOC).pdf $(MAIN).pdf $(DOC).*.pdf; true
	rm -Rf main-blx.bib
	rm -Rf .DS_Store; true
	rm -Rf .iTeXMac; true
	rm -Rf *.*.gz; true
	rm -Rf *.pdfsync; true
	rm -Rf *.synctex; true

desvn:
	find . -type d -name .svn -exec rm -rf {} +

#ARTIFACTS := $(shell find artifact)

#artifact: ${ARTIFACTS}
#	COPYFILE_DISABLE=1 tar -cvf artifact.tar artifact
#	gzip artifact.tar

# PACKAGING

DEP_TEX := $(shell find . \
	-not \( -path ./old-sections -prune \) \
	-not \( -path ./supplemental -prune \) \
	-not \( -path ./ijcai2018-formatting-guidelines -prune \) \
	-not \( -path ./arXiv -prune \) \
	-not \( -path ./formatting_instructions -prune \) \
	-not \( -path ./styles -prune \) \
	-name '*.tex' \
	)

DEP_TEX2 := $(DEP_TEX:%=arXiv/%)

arXiv/%.tex: %.tex
	latexpand --empty-comments $< > arXiv/$<
	sed -e '/^\s*%/d' -i '' arXiv/$<

arXiv:
	mkdir arXiv
	mkdir arXiv/figures

$(MAIN).bbl: $(DOC).arXiv.pdf

bundle: $(MAIN).bbl arXiv $(DEP_TEX:%=arXiv/%) ijcai18.sty
	cp -R $(MAIN).bbl ijcai18.sty arXiv
	cp -R $(DEP_FIGS) arXiv/figures
	(echo "\def\\\\arXiv{}\n"; cat arXiv/$(MAIN).tex) \
           > arXiv/$(MAIN).tex.temp
	mv arXiv/$(MAIN).tex.temp arXiv/$(MAIN).tex
	tar -cvf arXiv.tar arXiv
	gzip arXiv.tar

rebundle:
	rm -Rf arXiv; true
	rm -Rf arXiv.tar.gz; true
	make bundle


==> mc_on_attention_graph.tex <==
\begin{table}[t]
\centering
\begin{tabular}{llccccc}
	\toprule
	Task         & $\lg|\mathcal{P}^a|$ & $\text{C}^a_+$ & $\text{C}^a_-$&  $|\gamma_a(\pi^a_+)|/|\mathcal{P}^a|$ & acc.($\pi^a_+$)  &  acc.(rand.)\\ 
	\midrule
	\textbf{SVA} &                         &              &        &      &                                        &                         \\
	Obj.         & 27.6                   & 0.22         & 0.16   &   2.0e-7    &  0.74                                &   0.51              \\
	Subj.        & 27.6                    & 0.18         & 0.17   &  2.0e-7    & 0.56                                   &   0.49                 \\
	WSC          & 27.0                    & 0.16         & 0.24   &  1.8e-7    & 0.69                                   &   0.49                 \\
	APP          & 27.6                    & 0.18         & 0.15   &  1.6e-7    & 0.62                                  &   0.60                \\
	\midrule
	\textbf{RA}  &                         &              &        &       &                                        &                        \\
	NA           & 27.6                    & 0.18         & 0.18   &  1.4e-7    & 0.49                                  &    0.52                \\
	GA           & 28.6                    & 0.14         & 0.15   &  1.4e-7    & 0.72                                  &    0.55                 \\
	\bottomrule
\end{tabular}
\caption{Similar results of concentration and model compression as in Table \ref{tab:emb_qual}, using attention-level patterns $\pi^a$.}
\label{tab:attn_qual}
\end{table}

==> mc_on_embedding_graph.tex <==
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l }
% Task & L & $|P_{emb}|$ & \makecell{Emb\\ path} & $|P_{attn}|$ & \makecell{Attn\\ path} & \makecell{attn/skip} & $|N|$ & \makecell{MC.} & \makecell{rand} & Acc.  \\
% \hline
% \hline
% SVA & & & & & & & & &\\
% Obj. Relative & 11&1.8e+06&.34/.29&9.4e+11&.22/.16&.22/.23&.52&.99&.5 & \\
% Subj. Relative & 11&1.8e+06&.3/.31&9.4e+11&.18/.17&.22/.23&.55&.74&.5 & \\
% Within Sent. Comp& 10&1.e+06&.27/.38&5.3e+11&.16/.24&.22/.23&.48&1.0&.52 & \\
% Across PP & 11&1.8e+06&.33/.31&9.4e+11&.18/.15&.23/.24&.51&.92&.55 & \\

%  \hline
%  \hline
% Reflexive Anaphora & & & & & & & \\
% Number Agreement & 11&1.8e+06&.31/.32&9.4e+11&.18/.18&.23/.23&.49&.68&.54 &\\
% Gender Agreement & 13&4.8e+06&.22/.23&2.6e+12&.14/.15&.22/.22&.42&.76&.65 &\\
% \end{tabular}%

% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{.4}

% \newcolumntype{R}[2]{%
%     >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}%
%     l%
%     <{\egroup}%
% }
% \newcommand*\rot{\multicolumn{1}{R{60}{.7em}}}% no optional argument here, please!

% \begin{table}[t]
% \centering
% \begin{tabular}{llcccccc||cccccc}
% % 	\toprule
% 	\rot{Task}        & \rot{$\lg|\mathcal{P}^e|$} & \rot{$\text{C}^{\pi^e}_+$} & \rot{$\text{C}^{\pi^e}_-$}&  \rot{$|\gamma_e(\pi^e_+)|/|\mathcal{P}^e|$} & \rot{acc.($\pi^e_+$)}  & \rot{acc.(ori.)} & \rot{acc.(rand.)} & \rot{$\lg|\mathcal{P}^a|$} & \rot{ $\text{C}^{\pi^a}_+$} & \rot{$\text{C}^{\pi^a}_-$}&  \rot{$|\gamma_a(\pi^a_+)|/|\mathcal{P}^a|$ }&\rot{ acc.($\pi^a_+$)}  &  \rot{acc.(rand.)}\\ 
% 	\midrule
% 	\textbf{SVA} &                         &              &        &      &                                        &            &  &  &  & &           \\
% 	Obj.         & 14.4                    & .34         & .29   &  .06    & .99                                   &   .96        & .50  & 27.6                   & .22         & .16   &   2.0e-7    &  .74    &   .51   \\
% 	Subj.        & 14.4                    & .30         & .31   &  .09    & .74                                   &   1.00         & .50  & 27.6                    & .18         & .17   &  2.0e-7    & .56                                   &   .49        \\
% 	WSC          & 13.8                    & .27         & .38   &  .03    & 1.00                                   &   1.00         & .52    & 27.0                    & .16         & .24   &  1.8e-7    & .69                                   &   .49      \\
% 	APP          & 14.4                    & .33         & .31   &  .06    & .92                                  &   1.00         & .55   & 27.6                    & .18         & .15   &  1.6e-7    & .62                                  &   .60      \\
% 	\midrule
% 	\textbf{RA}  &                         &              &        &       &                                        &            &             \\
% 	NA           & 14.4                    & .31         & .32   &  .04    & .68                                   &    .83        & .54    & 27.6                    & .18         & .18   &  1.4e-7    & .49                                  &    .52     \\
% 	GA           & 15.4                    & .22         & .23   &   .02   & .76                                   &    .73         & .65    & 28.6                    & .14         & .15   &  1.4e-7    & .72                                  &    .55    \\
% 	\bottomrule
% \end{tabular}
% \caption{Concentration and compressed accuracy for Embedding-level Patterns $\pi^e$. $\text{C}^{\pi^e}_+$ \& $\text{C}^{\pi^e}_-$: The percentage of positive/negative embedding-level pattern influence over positive/negative input influence. $\mathcal{P}^e$: a set of all paths (reachable by GPR) from input to QoI. $\mathcal{\pi}^e_+$: embedding-level patterns for positively influential words. acc.(ori.) and  acc.(rand.) are the accuracies of the original model and a randomly compressed model which retains the same number of nodes as $\mathcal{\pi}^e_+$. }
% \label{tab:emb_qual}
% \end{table}

\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}

\begin{table}[h]
\centering
\resizebox{0.9\linewidth}{!}{%
    \begin{tabular}{c|cccc|cc}
    \hline
     \multirow{2}{*}{Task} & \multicolumn{4}{c}{SVA}& \multicolumn{2}{c}{RA}\\
     \cline{2-7}
     & Obj. & Subj. & WSC. & APP &  NA. & GA. \\
      \hline
     $C^{\positivepatterns^e}$ & .33& .30 &.27 &.33 &.31 &.22 \\
     $C^{\negativepatterns^e}$ &.29 &.30 &.38 &.31 &.31 &.23 \\
     $|\gamma_a(\positivepatterns^e)|/|\mathcal{P}^e|$ & .06 &.09 &.03 &.06 &.04 &.02 \\
     \hline
     acc.($\Pi^e_{+}$) &\textbf{.78} &\textbf{.80} &\textbf{1.0} &\textbf{.91} &\textbf{.80} &\textbf{.78} \\
     acc.($\Pi^e_{r}$) &.56 &.58 &.52 &.52 &.56 &.57 \\
     acc.($\baselinepatterns$) &.52&.50 &.53 &.61 &.52 &.68  \\
    \hline
     \hline
     $C^{\positivepatterns^a}$ &.21 &.18 &.16 &.18 &.18 &.14 \\
     $C^{\negativepatterns^a}$ &.17 &.16 &.25 &.15 &.17 &.15 \\
     $|\gamma_a(\positivepatterns^a)|/|\mathcal{P}^a|$ &\multirow{2}{*}{1.8} &\multirow{2}{*}{1.7}&\multirow{2}{*}{1.6} &\multirow{2}{*}{1.5} &\multirow{2}{*}{1.3} &\multirow{2}{*}{1.3} \\
     $(\cdot 10^{-6})$ & & & & & &  \\ 
     \hline
     $\mathcal{P}_{k,k'}$ &.58 &.57 &.57 & .59 &.46 &.53\\
     \hline
     acc.($\Pi^a_{+}$) &\textbf{.72} &\textbf{.58} &\textbf{.66} &\textbf{.66} &\textbf{.76} &\textbf{.69} \\
     acc.($\Pi^a_{r}$) &.52 &.50 &.49 &.49 &.46 &.48 \\
    %  acc.($\pi^a_{baseline,i}$) & & & & & & \\
    \hline
    acc.(ori.) &.96 &1.0 &1.0 &1.0 &.83 &.73 & 0.92 \\
    \end{tabular}}
    \caption{Pattern sufficiency, sparsity, and related metrics on various linguistic tasks. With $*\in \{e,a\}$, denoting embedding-level or attention-level metrics, respectively: $\text{C}^{\Pi^*_+}$, $\text{C}^{\Pi^*_-}$: positive/negative concentrations; $|\gamma_*(\Pi^*_{+})|/|\mathcal{P}^*|$: proportion of paths contained in the abstracted patterns over the total number of paths in the corresponding graph; $\mathcal{P}_{k,k'}$: probability that the attention head nodes in $\Pi^a$ are actually the head (among 8) with largest attention weight; acc.($\Pi^*_{+}$), acc.($\Pi^*_{r}$), acc.($\baselinepatterns$) are compressed accuracy of the the positive patterns and two baseline patterns, respectively. \todo{Replace some symbols with words to better corefer to results and their sections in the discussion.}}
\label{tab:emb_qual}
% \vspace{-5pt}
\end{table}

% \begin{table*}[ht]
% \begin{minipage}[b]{0.7\linewidth}
% % \centering
%         \resizebox{0.9\linewidth}{!}{%

%         \begin{tabular}{c|cc|cc|cc|cc|cc|cc|c}
%         \hline
%         \multirow{2}{*}{Task} & \multicolumn{2}{c}{$C^{\positivepatterns^*}$} &
%         \multicolumn{2}{c}{$C^{\negativepatterns^*}$} & \multicolumn{2}{c}{$\frac{|\gamma_*(\pi^*_{+})|}{|\mathcal{P}^*|}$} & 
%         \multicolumn{2}{c}{A($\pi^*_{+}$)} & 
%         \multicolumn{2}{c}{A($\pi^*_{r}$)} & 
%         \multicolumn{2}{c}{A($\pi_{b}$)} & 
%         \multirow{2}{*}{A(ori.)} \\
%         \cline{2-13}
%         &$e$ & $a$ & $e$ & $a$ & $e$ & $a$ & $e$ & $a$ & $e$ & $a$ & $b_1$ & $b_2$ &  \\
%         \hline
%         \textbf{SVA} & & & & & & & & & & & &\\
%         \text{Obj.} & .33&.21 & .29&.17 &.06 &1.8e-6 &.78 &.72 &.56 &.52& &.52 & .96\\
%         \text{Subj.} & .30&.18 &.30 &.16 &.09 &1.7e-6 &.80 &.58 &.58 &.50& &.52 & 1.00\\
%         \text{WSC} &.27 &.16 &.38 &.25  &.03 &1.6e-6 &1.0&.66 &.52 &.49& &.53 & 1.00\\
%         \text{APP} &.33 &.18 &.31 &.15  &.06 &1.5e-6 &.91 &.66&.52 &.49& &.61 & 1.00\\
%         \textbf{RA} & & & & & & & & & & & &\\
%         \text{NA} &.31 &.18 &.31 &.17 &.04 &1.3e-6 &.80 &.76 &.56 &.46& &.52 & .83\\
%         \text{GA}  &.22 &.14 &.23 &.15 &.02 &1.3e-6 &.78 &.69 &.57&.48& &.68 & .73\\
%         \end{tabular}}
%     \caption{\update{Pattern sufficiency, sparsity, and related metrics on various linguistic tasks. Metrics are shown in the \nth{1} row while the \nth{2} row indicate graph levels: $*$ denotes $e$ or $a$, corresponding to abstracted embedding-level patterns $\pi^e$ or attention-level patterns $\pi^a$, respectively. $lg|\mathcal{P}^*|$: natural log of the number of possible paths; $\text{C}^{\Pi^*}_+$, $\text{C}^{\Pi^*}_-$: positive/negative concentrations; $\frac{|\gamma_*(\pi^*_{+})|}{|\mathcal{P}^*|}$: percentage of paths in the abstracted patterns over the total number of paths; acc.($\pi^*_{+}$): the compressed accuracy of abstracted patterns; acc.(rand. $*$): the compressed accuracy of randomly compressed models; acc.(ori.): the accuracy of the original model $\text{BERT}_{\text{SMALL}}$.} \pxm{The path counts seem like they are for a single input word to a single qoi, not all combinations of paths.}}
%     \label{tab:emb_qual}
% \end{minipage}\hfill
% \begin{minipage}[b]{0.3\linewidth}
% \centering
% \includegraphics[width=40mm]{example-image}
% \captionof{figure}{2-D scatterplot of the Student Database}
% \label{fig:image}
% \end{minipage}
% \end{table*}

% \begin{table*}[ht]
% %  \begin{minipage}{\textwidth}

% %   \begin{minipage}[b]{0.49\linewidth}
%     % \begin{table}[t]
%         % \centering
%         \resizebox{.6\textwidth}{!}{%
%         \begin{tabular}{c|cc|cc|cc|cc|cc|cc|c}
%         \hline
%         \multirow{2}{*}{Task} & \multicolumn{2}{c}{$lg|\mathcal{P}^*|$} & \multicolumn{2}{c}{$C^{\positivepatterns^*}$} &
%         \multicolumn{2}{c}{$C^{\negativepatterns^*}$} & \multicolumn{2}{c}{$\frac{|\gamma_*(\pi^*_{+})|}{|\mathcal{P}^*|}$} & 
%         \multicolumn{2}{c}{acc.($\pi^*_{+}$)} & 
%         \multicolumn{2}{c}{acc.(rand. $*$)} & 
%         \multirow{2}{*}{acc.(ori.)} \\
%         \cline{2-13}
%         &$e$ & $a$ & $e$ & $a$ & $e$ & $a$ & $e$ & $a$ & $e$ & $a$ & $e$ & $a$ &  \\
%         \hline
%         \textbf{SVA} & & & & & & & & & & & &\\
%         \text{Obj.} & 14.4&27.6 & .34&.22 & .29&.16 &.06 &2.0e-7 &.99 &.74 &.50 &.51&.96\\
%         \text{Subj.} &14.4 &27.6 & .30&.18 &.31 &.17 &.09 &2.0e-7 &.74 &.56 &.50 &.49&1.00\\
%         \text{WSC} & 13.8& 27.0&.27 &.16 &.38 &.24  &.03 &1.8e-7 &1.00&.69 &.52 &.49&1.00\\
%         \text{APP} & 14.4&27.6 &.33 &.18 &.31 &.15  &.06 &1.6e-7 &.92 &.62&.55 &.60&1.00\\
%         \textbf{RA} & & & & & & & & & & & &\\
%         \text{NA} &14.4 &27.6 &.31 &.18 &.32 &.18 &.04 &1.4e-7 &.68 &.49 &.54 &.52&.83\\
%         \text{GA} & 15.4&28.6 &.22 &.14 &.23 &.15 &.02 &1.4e-7 &.76 &.72 &.65&.55&.73\\
%         \end{tabular}}
%     % \caption{\update{Pattern sufficiency, sparsity, and related metrics on various linguistic tasks. Metrics are shown in the \nth{1} row while the \nth{2} row indicate graph levels: $*$ denotes $e$ or $a$, corresponding to abstracted embedding-level patterns $\pi^e$ or attention-level patterns $\pi^a$, respectively. $lg|\mathcal{P}^*|$: natural log of the number of possible paths; $\text{C}^{\Pi^*}_+$, $\text{C}^{\Pi^*}_-$: positive/negative concentrations; $\frac{|\gamma_*(\pi^*_{+})|}{|\mathcal{P}^*|}$: percentage of paths in the abstracted patterns over the total number of paths; acc.($\pi^*_{+}$): the compressed accuracy of abstracted patterns; acc.(rand. $*$): the compressed accuracy of randomly compressed models; acc.(ori.): the accuracy of the original model $\text{BERT}_{\text{SMALL}}$.} \pxm{The path counts seem like they are for a single input word to a single qoi, not all combinations of paths.}
%     % \label{tab:emb_qual}
%     % \end{table}
%     % \end{minipage}
     
%      \hfill

%      \begin{minipage}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[width=40mm]{images/completeness.png}
%       \end{minipage}
% %   \end{minipage}
% \end{table*}  
% \begin{table}[t]
%     % \centering
%     \resizebox{.48\textwidth}{!}{%
%     \begin{tabular}{c|cc|cc|cc|cc|c}
%     \hline
%     \multirow{2}{*}{Task}  & \multicolumn{2}{c}{$C^{\positivepatterns^*}$} & \multicolumn{2}{c}{$\frac{|\gamma_*(\pi^*_{+})|}{|\mathcal{P}^*|}$} & 
%     \multicolumn{2}{c}{acc.($\pi^*_{+}$)} & 
%     \multicolumn{2}{c}{acc.($\pi^*_{r}$)} & 
    
%     \multirow{2}{*}{acc.(ori.)} \\
%     \cline{2-9}
%     & $e$ & $a$ & $e$ & $a$ & $e$ & $a$ & $e$ & $a$ &  \\
%     \hline
%     \textbf{SVA}  & & & & & & & & &\\
%     \text{Obj.}  & .34&.22  &.06 &2.0e-7 &.99 &.74 &.50 &.51&.96\\
%     \text{Subj.}  & .30&.18 &.09 &2.0e-7 &.74 &.56 &.50 &.49&1.0\\
%     \text{WSC} &.27 &.16 &.03 &1.8e-7 &1.0    &.69 &.52 &.49&1.0\\
%     \text{APP}  &.33 &.18 &.06 &1.6e-7 &.92 &.62&.55 &.60&1.0\\
%     \textbf{RA}  & & & & & & & & &\\
%     \text{NA}  &.31 &.18 &.04 &1.4e-7 &.68 &.49 &.54 &.52&.83\\
%     \text{GA}  &.22 &.14 &.02 &1.4e-7 &.76 &.72 &.65&.55&.73\\
%     \end{tabular}}
% \caption{\update{Pattern sufficiency, sparsity, and related metrics on various linguistic tasks. Metrics are shown in the \nth{1} row while the \nth{2} row indicate graph levels: $*$ denotes $e$ or $a$, corresponding to abstracted embedding-level patterns $\pi^e$ or attention-level patterns $\pi^a$, respectively. $\text{C}^{\Pi^*}_+$: positive concentrations; $\frac{|\gamma_*(\pi^*_{+})|}{|\mathcal{P}^*|}$: percentage of paths in the abstracted patterns over the total number of paths; acc.($\pi^*_{+}$): the compressed accuracy of abstracted patterns; acc.(rand. $*$): the compressed accuracy of randomly compressed models; acc.(ori.): the accuracy of the original model $\text{BERT}_{\text{SMALL}}$.} \pxm{The path counts seem like they are for a single input word to a single qoi, not all combinations of paths.}}
% \label{tab:emb_qual}
% \end{table}


%\vspace{.25cm}



% \todo. $\downarrow$acc.($\cdot$): drop of accuracy compared with the original model if only positive paths ($\mathcal{P}^+_e$) or the embedding-level significant path ($\pi^e$) are retained. $\uparrow$acc.($\cdot$): increase of accuracy if only $\mathcal{P}^+_e$ or $\pi^e$ are retained compared with retaining random paths }



% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l }
% 	Task & L & $|P_{emb}|$ & \makecell{Emb\\ path} & $|P_{attn}|$ & \makecell{Attn\\ path} & \makecell{attn/skip} & $|N|$ & \makecell{MC.} & \makecell{rand} & Acc.  \\
% 	\hline
% 	\hline
% 	SVA & & & & & & & & &\\
% 	Obj. Relative & 11&1.8e+06&.34/.29&9.4e+11&.22/.16&.22/.23&.52&.99&.5 & \\
% 	Subj. Relative & 11&1.8e+06&.3/.31&9.4e+11&.18/.17&.22/.23&.55&.74&.5 & \\
% 	Within Sent. Comp& 10&1.e+06&.27/.38&5.3e+11&.16/.24&.22/.23&.48&1.0&.52 & \\
% 	Across PP & 11&1.8e+06&.33/.31&9.4e+11&.18/.15&.23/.24&.51&.92&.55 & \\
	
% 	 \hline
% 	 \hline
% 	Reflexive Anaphora & & & & & & & \\
% 	Number Agreement & 11&1.8e+06&.31/.32&9.4e+11&.18/.18&.23/.23&.49&.68&.54 &\\
% 	Gender Agreement & 13&4.8e+06&.22/.23&2.6e+12&.14/.15&.22/.22&.42&.76&.65 &\\
% \end{tabular}%


==> metrics.tex <==

% \indent\textbf{Concentration.} Given a sentence $\xvec$, the positive and negative concentration $\text{C}_+$ and $\text{C}_-$ are
% the percentages of the influence flowing through total positive or negative $\pi^e_i$ and $\pi^a_i$, over the total positive or negative influence, respectively.\caleb{might be a bit confusing, adapt with math
%   notations?} We also calculate the proportion of all paths within the positive patterns over all paths from input to QoI, $|\gamma_e(\pi^e_+)|/|\mathcal{P}^e|$ and $|\gamma_a(\pi^a_+)|/|\mathcal{P}^a|$.
% %, where $0 \leq \text{C}^+, \text{C}^- \leq 1$ (see discussion in Appendix~\ref{appendix: path
% %influence}).
% Based on the conservation of pattern influence,  high concentration suggests that a large portion of distributional influence flows across significant
% patterns, instead of sparely distributed over a large number of paths. 

% (e.g. the number of total
% paths in an embedding-level graph is more than $2^{14}$ for a sentence with 11 tokens).

\noindent\textbf{Model Compression.}
% We validate the significane of the paths by only keeping the paths $\pi^e$ or $\pi^a$ returned by
% GPR and replace the output of other nodes as the $\hvec^0_m$, the input embedding of
% \texttt{[MASK]}, during the inference time. In the other words, the model is ``compressed" down.
% We compare the accuracy of a ``compressed" model on all tasks mentioned above against the
% original model and a model retaining randomly sampled paths. Input attributions such as II used
% in this paper has been shown to be feasible though ablating the input features of low influence
% \todo{citation}.
To validate that the extracted patterns are actually significant for abstracting a specific concept
from the input embedding to the output QoI, we employ a model compression algorithm inspired by \citet{DBLP:conf/acl/LuMLFD20}. 
For each example, we only retain the nodes from $\pi^e_+$ or $\pi^a_+$ while replacing all other nodes, layer by layer. 
Starting from the first layer, \caleb{not sure if the notion of layer is clear here, since they are different for embedding-level and attention-level graphs}the embedding nodes not in $\pi^e_+$  (or the attention/skip connection
nodes not in $\pi^a_+$) are replaced by the embedding of \texttt{[MASK]} (zero vectors for attention/skip
nodes), while the nodes in $\pi^e_+$ or $\pi^a_+$ will remain untouched. The retained and replaced node
together will be forwardly passed to the next layer using the original model parameters until a new set of nodes needs to be retained or replaced. 
\caleb{would it be better to show with an example? or the diagram in Figure 2}

% \noindent\textbf{Concentration \& Spread of MP} The positive/negative concentration of a EMPI(or
% AMPI) in a graph is defined as the sum of all positive/negative EMPI(or AMPI) over the sum of all
% positive/negative II. \todo{definition or description?} As is shown in table \ref{tab:qual_data},
% EMPI account for a large portion of both positive and negative influence, across all examples,
% ranging from 22\% to 34\% of total II. Within the EMPI through GPR, the extracted AMPI also
% account for a great proportion, ranging from 14\% to 24\% of total II. This percentage is really
% siginifcany compared to the number of gradient paths in a EMP or AMP, which is shown by log scale
% in \ref{tab:qual_data}. The concentration also shows that although the other part of the model
% may also carry a large percentage of the influence, within an extracted EMP, most of the
% influence in EMPI is concentrated either to a single attention head or the skip connection.
% \caleb{this is quite similar to the conclusions in the ACL paper, should I mention?}

% % \todo{caleb: A table showing the concentration stats}
% % \todo{how much does skip connection accounted for(Expected value)}

% \noindent\textbf{Model Compression}\caleb{Use pseudo-code and stricter definitions or
% description?} Input attributions such as II used in this paper has been shown to be feasible
% though ablating the input features of low influence \todo{citation}. However, to verify that the
% extracted MPs are actually significant for transmitting the information from the input embedding
% to the output QoI, we employ a model compression algorithm, inspired by those used in
% \citet{DBLP:conf/acl/LuMLFD20}. Since there is no way to only retain the portion of extracted MPs
% in forward pass, we propose an approximating model compression procedure: for each example, we
% only retain the nodes where positive MPs pass through while ``churning'' the nodes where no
% positive MPs pass though. The ``churning'' and ``retaining'' operations are conducted in the
% input layer, and as each layer's output embedding is calculated. In each layer, the embedding
% nodes to be churned will be replaced by the ``mask embedding'', while the nodes to be retained
% will remain untouched. The retained and churned node together will be plugged as inputs to the
% next layer.


==> sec_eval_conc_table.tex <==
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1}

% \begin{table}[!t]
% \centering
% \resizebox{0.45\linewidth}{!}{%
%     \begin{tabular}{c|cccc|cc}
%     \hline
%      \multirow{2}{*}{Task} & \multicolumn{4}{c}{SVA}& \multicolumn{2}{c}{RA}\\
%      \cline{2-7}
%      & Obj. & Subj. & WSC & APP &  NA & GA \\
%       \hline
%      conc.(${\positivepatterns^e}$) & .33& .30 &.27 &.33 &.31 &.22 \\
%      conc.(${\negativepatterns^e}$) &.29 &.30 &.38 &.31 &.31 &.23 \\
%      sparsity(${\positivepatterns^e}$) & .06 &.09 &.03 &.06 &.04 &.02 \\
%     %  $|\gamma_a(\positivepatterns^e)|/|\mathcal{P}^e|$ & .06 &.09 &.03 &.06 &.04 &.02 \\
%     \hline
%      conc.(${\positivepatterns^a}$) &.21 &.18 &.16 &.18 &.18 &.14 \\
%      conc.(${\negativepatterns^a}$) &.17 &.16 &.25 &.15 &.17 &.15 \\
%      sparsity(${\positivepatterns^a}$) &\multirow{2}{*}{1.8} &\multirow{2}{*}{1.7}&\multirow{2}{*}{1.6} &\multirow{2}{*}{1.5} &\multirow{2}{*}{1.3} &\multirow{2}{*}{1.3} \\
%      $(\cdot 10^{-6})$ & & & & & &  \\ 
%     %  \hline
%     %  $\mathcal{P}_{k,k'}$ &.58 &.57 &.57 & .59 &.46 &.53\\
%     %  \hline
%     \end{tabular}}
%     \caption{Sparsity related metrics: conc.(${\positivepatterns^*}$), conc.(${\negativepatterns^*}$): positive/negative concentrations; sparsity(${\allpatterns^*}$): proportion of paths contained in the abstracted patterns over the total number of paths in the corresponding graph.}
% \label{tab:emb_qual}
% \end{table}








% \todo. $\downarrow$acc.($\cdot$): drop of accuracy compared with the original model if only positive paths ($\mathcal{P}^+_e$) or the embedding-level significant path ($\pi^e$) are retained. $\uparrow$acc.($\cdot$): increase of accuracy if only $\mathcal{P}^+_e$ or $\pi^e$ are retained compared with retaining random paths }



% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l }
% 	Task & L & $|P_{emb}|$ & \makecell{Emb\\ path} & $|P_{attn}|$ & \makecell{Attn\\ path} & \makecell{attn/skip} & $|N|$ & \makecell{MC.} & \makecell{rand} & Acc.  \\
% 	\hline
% 	\hline
% 	SVA & & & & & & & & &\\
% 	Obj. Relative & 11&1.8e+06&.34/.29&9.4e+11&.22/.16&.22/.23&.52&.99&.5 & \\
% 	Subj. Relative & 11&1.8e+06&.3/.31&9.4e+11&.18/.17&.22/.23&.55&.74&.5 & \\
% 	Within Sent. Comp& 10&1.e+06&.27/.38&5.3e+11&.16/.24&.22/.23&.48&1.0&.52 & \\
% 	Across PP & 11&1.8e+06&.33/.31&9.4e+11&.18/.15&.23/.24&.51&.92&.55 & \\
	
% 	 \hline
% 	 \hline
% 	Reflexive Anaphora & & & & & & & \\
% 	Number Agreement & 11&1.8e+06&.31/.32&9.4e+11&.18/.18&.23/.23&.49&.68&.54 &\\
% 	Gender Agreement & 13&4.8e+06&.22/.23&2.6e+12&.14/.15&.22/.22&.42&.76&.65 &\\
% \end{tabular}%

